Learning from Sets of Items in Recommender Systems

Most of the existing recommender systems use the ratings provided by users on individual items. An additional source of preference information is to use the ratings that users provide on sets of items. The advantages of using preferences on sets are two-fold. First, a rating provided on a set conveys some preference information about each of the set's items, which allows us to acquire a user's preferences for more items that the number of ratings that the user provided. Second, due to privacy concerns, users may not be willing to reveal their preferences on individual items explicitly but may be willing to provide a single rating to a set of items, since it provides some level of information hiding. This paper investigates two questions related to using set-level ratings in recommender systems. First, how users' item-level ratings relate to their set-level ratings. Second, how collaborative filtering-based models for item-level rating prediction can take advantage of such set-level ratings. We have collected set-level ratings from active users of Movielens on sets of movies that they have rated in the past. Our analysis of these ratings shows that though the majority of the users provide the average of the ratings on a set's constituent items as the rating on the set, there exists a significant number of users that tend to consistently either under- or over-rate the sets. We have developed collaborative filtering-based methods to explicitly model these user behaviors that can be used to recommend items to users. Experiments on real data and on synthetic data that resembles the under- or over-rating behavior in the real data, demonstrate that these models can recover the overall characteristics of the underlying data and predict the user's ratings on individual items.

==> notation.tex <==
%!TEX root = paper.tex
Throughout the paper, all vectors are column vectors and are represented by
bold lowercase letters (e.g., $\bm{p,q}$). The row vectors are represented by
having the transpose super-script (e.g., $\bm{p^T}$). Matrices are represented by upper
case letters (e.g., ${R,W}$). The ($i$, $j$) entry of matrix $W$ is denoted by
$w_{i,j}$. The \textit{i}th row of matrix $P$ is represented by $\bm{p}_i^T$. We use calligraphic letters to denote sets (e.g.,
$\mathcal{C,D}$), and the size of a set $\mathcal{S}$ is represented by
$|\mathcal{S}|$. 




